Mercury: QoS-Aware Tiered Memory System

Memory tiering has received wide adoption in recent years as an effective solution to address the increasing memory demands of memory-intensive workloads. However, existing tiered memory systems often fail to meet service-level objectives (SLOs) when multiple applications share the system because they lack Quality-of-Service (QoS) support. Consequently, applications suffer severe performance drops due to local memory contention and memory bandwidth interference. In this paper, we present Mercury, a QoS-aware tiered memory system that ensures predictable performance for coexisting memory-intensive applications with different SLOs. Mercury enables per-tier page reclamation for application-level resource management and uses a proactive admission control algorithm to satisfy SLOs via per-tier memory capacity allocation and intra- and inter-tier bandwidth interference mitigation. It reacts to dynamic requirement changes via real-time adaptation. Extensive evaluations show that Mercury improves application performance by up to 53.4% and 20.3% compared to TPP and Colloid, respectively.

==> observation.tex <==
\section{QoS Analysis in Tiered Memory}
\label{sec:observation}
\jiaheng{move this to the beginning of section 2, and section 3 is mercury}
In this section, we quantitatively analyze how local memory contention and memory bandwidth interference affect application performance and draw key insights to design \name{}.
All results are collected on the same CXL-based tiered memory system as in Section~\ref{sec:lack-of-qos}.

\begin{figure}[!t]
    \centering
    \subfloat[Impact on Latency Performance]{
        \label{fig:moti-lt-sweep}
        \includegraphics[width=3in]{Figures/Moti/moti_lt_sweep.pdf}
    } \\
    \subfloat[Impact on Bandwidth Performance]{
        \label{fig:moti-bw-sweep}
        \includegraphics[width=3in]{Figures/Moti/moti_bw_sweep.pdf}
    }
    \captionsetup{width=\columnwidth}
    \caption{Latency and bandwidth performance at different CXL interleaving ratios to illustrate the impact of local memory.}%
    \label{fig:moti-local-memory-impact}
\end{figure}

\subsection{Impact of Available Local Memory}
\label{sec:local-memory-impact}
We start by studying the impact of available local memory on application performance, as applications can easily run short of local memory during memory contention.
We develop two microbenchmarks to represent LS and BI applications, which we denote as \textit{LS} and \textit{BI} in Section~\ref{sec:observation} for brevity.
\textit{LS} performs random memory access among a 4GB memory region.
\textit{BI} allocates enough CPU cores to generate memory bandwidth at maximum capacity on 128MB region per core.
These microbenchmarks allow us to easily control the proportion of memory access on CXL memory (the rest goes to local memory), which we denote as the CXL interleaving percentage.
Figure~\ref{fig:moti-local-memory-impact} shows the impact of available local memory on latency and bandwidth performance by varying the CXL interleaving ratio of the two microbenchmarks.
We observe the memory access latency of \textit{LS} is proportional to its available local memory, and it becomes 2$\times$ slower when all memory is moved to CXL in the worst case.
On the other hand, \textit{BI}'s bandwidth performance degrades as more memory is accessed from CXL, dropping to 25\% of its original performance when all memory is accessed via CXL.
\begin{tcolorbox}[width=\linewidth, boxsep=0pt, left=5pt, right=5pt, sharp corners=all, colback=white!92!black, boxrule=1pt, frame empty]
\textbf{Takeaway \#1}: Local memory directly affects the performance of both types of applications and should be allocated judiciously during memory contention.
\end{tcolorbox}

\subsection{Deep Dive in Memory Interference}
\label{sec:inter-tier-interference}

\begin{figure}[!t]
    \centering
    \includegraphics[width=3in]{Figures/Moti/moti_lt_local_bw_sweep.pdf}%
    \captionsetup{width=\columnwidth}
    \caption{Performance of \textit{LS} when \textit{BI} is generating bandwidth at different CXL interleaving percentage. Migrating \textit{BI} to CXL does not always lead to better performance of \textit{LS} due to inter-tier interference. \textit{BI}'s performance is very close to Figure~\ref{fig:moti-bw-sweep} and omitted in the interest of space.}%
    \label{fig:moti-lt-local-bw-sweep}
\end{figure}


We now take a close look at how LS applications are affected by memory bandwidth interference from BI applications. %

\para{Varying \textit{BI} across tiers.}
In this experiment, we configure \textit{LS} to always access local memory and vary \textit{BI}'s CXL-interleaving percentage.
The results are shown in Figure~\ref{fig:moti-lt-local-bw-sweep}, and we make two key observations.
First, as more bandwidth is generated on CXL, instead of a monotonic change, the performance of the LS application initially decreases and then increases.
Second, the interference becomes the worst when all memory bandwidth is generated from CXL, even though the total memory bandwidth is the lowest at this moment. 

\begin{figure}[!t]
    \centering
    \includegraphics[width=2.5in]{Figures/cxl_arch2.pdf}%
    \captionsetup{width=\columnwidth}
    \caption{Architectural diagram of how memory requests are handled in CXL-based tiered memory.}%
    \label{fig:cxl-arch}
\end{figure}
To explain the behavior in the last experiment, we need to understand how memory requests are handled in a tiered memory system.
Figure~\ref{fig:cxl-arch} presents a high-level diagram.
There exist separate fixed-size queues in the hardware for memory requests to/from local and CXL memory.
Initially, when bandwidth on local memory is high, its corresponding queue fills up, causing interference on local memory (i.e., intra-tier interference) to dominate.
When \textit{BI} starts to move requests from local memory to CXL, intra-tier interference decreases, causing latency to drop.
When more requests are moved to the CXL side, the queue holding CXL requests builds up.
Since both types of requests are handled by the same set of CPU cores, busy processing of the CXL requests can slow down the concurrent requests for local memory. 
\begin{tcolorbox}[width=\linewidth, boxsep=0pt, left=5pt, right=5pt, sharp corners=all, colback=white!92!black, boxrule=1pt, frame empty]
\textbf{Takeaway \#2}: We should determine the right amount of memory to migrate BI applications that \textit{reduces intra-tier interference while keeping inter-tier interference low.}
\end{tcolorbox}


\begin{figure}[!t]
    \centering
    \includegraphics[width=3in]{Figures/Moti/moti_bw_local_lt_sweep.pdf}%
    \captionsetup{width=\columnwidth}
    \caption{Performance of \textit{LS} at different CXL interleaving ratios when \textit{BI} is fixed on local memory. Migrating more requests away from local memory does not improve performance as more requests are accessing the slower tier.}
    \label{fig:moti_bw_local_lat_sweep}
\end{figure}

\para{Varying \textit{LS} across tiers.}
Figure~\ref{fig:moti_bw_local_lat_sweep} shows the results of interference in a different setting, where we keep \textit{BI} fixed on local memory and vary \textit{LS}'s CXL interleaving percentage. %
This is used to simulate the scenario where one attempts to mitigate the interference on the fast tier by migrating \textit{LS}'s requests away from local memory to CXL memory.
However, such an approach leads to worse performance because more memory requests are now accessing the slow tier. \jiaheng{if we want to improve the performance of the LS app, the performance could not be improved much because of the heavy bandwidth interference. As a result, when we want to improve the performance of the LS app, we should always first mitigate the bandwidth interference}
\begin{tcolorbox}[width=\linewidth, boxsep=0pt, left=5pt, right=5pt, sharp corners=all, colback=white!92!black, boxrule=1pt, frame empty]
\textbf{Takeaway \#3}: We should proactively mitigate the interference on local memory to provide predictable performance for LS applications.
\end{tcolorbox}





